An Analysis of Variations in the Effectiveness of Query Performance Prediction

A query performance predictor estimates the retrieval effectiveness of an IR system for a given query. An important characteristic of QPP evaluation is that, since the ground truth retrieval effectiveness for QPP evaluation can be measured with different metrics, the ground truth itself is not absolute, which is in contrast to other retrieval tasks, such as that of ad-hoc retrieval. Motivated by this argument, the objective of this paper is to investigate how such variances in the ground truth for QPP evaluation can affect the outcomes of QPP experiments. We consider this not only in terms of the absolute values of the evaluation metrics being reported (e.g. Pearson's $r$, Kendall's $\tau$), but also with respect to the changes in the ranks of different QPP systems when ordered by the QPP metric scores. Our experiments reveal that the observed QPP outcomes can vary considerably, both in terms of the absolute evaluation metric values and also in terms of the relative system ranks. Through our analysis, we report the optimal combinations of QPP evaluation metric and experimental settings that are likely to lead to smaller variations in the observed results.

==> refs.tex <==
@book{hiemstra,
  author    = {Djoerd Hiemstra},
  title     = {Using language models for information retrieval},
  publisher = {Univ. Twente},
  year      = {2001},
  isbn      = {978-90-75296-05-1},
}

@article{ndcg,
author = {J\"{a}rvelin, Kalervo and Kek\"{a}l\"{a}inen, Jaana},
title = {Cumulated Gain-Based Evaluation of IR Techniques},
year = {2002},
issue_date = {October 2002},
publisher = {ACM},
address = {New York, NY, USA},
volume = {20},
number = {4},
issn = {1046-8188},
abstract = {Modern large retrieval environments tend to overwhelm their users by their large output.
Since all documents are not of equal relevance to their users, highly relevant documents
should be identified and ranked first for presentation. In order to develop IR techniques
in this direction, it is necessary to develop evaluation approaches and methods that
credit IR methods for their ability to retrieve highly relevant documents. This can
be done by extending traditional evaluation methods, that is, recall and precision
based on binary relevance judgments, to graded relevance judgments. Alternatively,
novel measures based on graded relevance judgments may be developed. This article
proposes several novel measures that compute the cumulative gain the user obtains
by examining the retrieval result up to a given ranked position. The first one accumulates
the relevance scores of retrieved documents along the ranked result list. The second
one is similar but applies a discount factor to the relevance scores in order to devaluate
late-retrieved documents. The third one computes the relative-to-the-ideal performance
of IR techniques, based on the cumulative gain they are able to yield. These novel
measures are defined and discussed and their use is demonstrated in a case study using
TREC data: sample system run results for 20 queries in TREC-7. As a relevance base
we used novel graded relevance judgments on a four-point scale. The test results indicate
that the proposed measures credit IR methods for their ability to retrieve highly
relevant documents and allow testing of statistical significance of effectiveness
differences. The graphs based on the measures also provide insight into the performance
IR techniques and allow interpretation, for example, from the user point of view.},
journal = {ACM Trans. Inf. Syst.},
month = oct,
pages = {422–446},
numpages = {25},
keywords = {cumulated gain, Graded relevance judgments}
}

@InProceedings{pmlr-v15-ravikumar11a,
  title = 	 {{On NDCG Consistency of Listwise Ranking Methods}},
  author = 	 {Ravikumar, Pradeep and Tewari, Ambuj and Yang, Eunho},
  booktitle = 	 {Proceedings of the Fourteenth International Conference on Artificial Intelligence and Statistics},
  pages = 	 {618--626},
  year = 	 {2011},
  volume = 	 {15},
  address = 	 {Fort Lauderdale, FL, USA},
  publisher =    {PMLR},
  abstract = 	 {We examine the consistency of listwise ranking methods with respect to the popular Normalized Discounted Cumulative Gain (NDCG) criterion. The most successful listwise approaches replace NDCG with a surrogate that is easier to optimize. We characterize NDCG consistent surrogates to discover a surprising fact: several commonly used surrogates are NDCG inconsistent. We then show how to change them so that they become NDCG consistent in a strong but natural sense. An explicit characterization of strong NDCG consistency is provided. Going beyond qualitative consistency considerations, we also give quantitive statements that enable us to transform the excess error, as measured in the surrogate, to the excess error in comparison to the Bayes optimal ranking function for NDCG. Finally, we also derive improved results if a certain natural “low noise"” or “large margin"” condition holds.  Our experiments demonstrate that ensuring NDCG consistency does improve the performance of listwise ranking methods on real-world datasets. Moreover, a novel surrogate function suggested by our theoretical results leads to further improvements over NDCG consistent versions of existing surrogates. [pdf][supplementary]}
}

@inproceedings{Xue,
author = {Xue, Xiaobing and Croft, W. Bruce},
title = {Automatic Query Generation for Patent Search},
year = {2009},
booktitle = {Proc. of CIKM},
pages = {2037–2040},
}

@inproceedings{Ganguly,
author = {Ganguly, Debasis and Leveling, Johannes and Magdy, Walid and Jones, Gareth J.F.},
title = {Patent Query Reduction Using Pseudo Relevance Feedback},
booktitle = {Proc. of CIKM},
pages = {1953–1956},
series = {CIKM ’11}
}

@inproceedings{TakakiFI04,
  author    = {Toru Takaki and
               Atsushi Fujii and
               Tetsuya Ishikawa},
  title     = {Associative document retrieval by query subtopic analysis and its
               application to invalidity patent search},
  booktitle = {Proc. of {CIKM'04}},
  pages     = {399--405},
  year      = {2004}
}

@inproceedings{maip_cikm,
author = {Yilmaz, Emine and Aslam, Javed A.},
title = {Estimating Average Precision with Incomplete and Imperfect Judgments},
year = {2006},
isbn = {1595934332},
publisher = {ACM},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1183614.1183633},
doi = {10.1145/1183614.1183633},
abstract = {We consider the problem of evaluating retrieval systems using incomplete judgment information. Buckley and Voorhees recently demonstrated that retrieval systems can be efficiently and effectively evaluated using incomplete judgments via the bpref measure [6]. When relevance judgments are complete, the value of bpref is an approximation to the value of average precision using complete judgments. However, when relevance judgments are incomplete, the value of bpref deviates from this value, though it continues to rank systems in a manner similar to average precision evaluated with a complete judgment set. In this work, we propose three evaluation measures that (1) are approximations to average precision even when the relevance judgments are incomplete and (2) are more robust to incomplete or imperfect relevance judgments than bpref. The proposed estimates of average precision are simple and accurate, and we demonstrate the utility of these estimates using TREC data.},
booktitle = {Proceedings of the 15th ACM International Conference on Information and Knowledge Management},
pages = {102–111},
numpages = {10},
keywords = {sampling, Bpref, evaluation, average precision, incomplete judgments},
location = {Arlington, Virginia, USA},
series = {CIKM '06}
}

@inproceedings{javed_aslam_ecir07,
author = {Aslam, Javed A. and Pavlu, Virgil},
title = {Query Hardness Estimation Using Jensen-Shannon Divergence among Multiple Scoring Functions},
year = {2007},
publisher = {Springer-Verlag},
address = {Berlin, Heidelberg},
booktitle = {Proceedings of the 29th European Conference on IR Research},
pages = {198–209},
numpages = {12},
location = {Rome, Italy},
series = {ECIR'07}
}

@inproceedings{kurland_qpp_rlm,
author = {Butman, Olga and Shtok, Anna and Kurland, Oren and Carmel, David},
title = {Query-Performance Prediction Using Minimal Relevance Feedback},
year = {2013},
booktitle = {Proceedings of the 2013 Conference on the Theory of Information Retrieval},
pages = {14–21},
series = {ICTIR '13}
}

@inproceedings{carmel_qpp_sigir10,
author = {Carmel, David and Yom-Tov, Elad},
title = {Estimating the Query Difficulty for Information Retrieval},
year = {2010},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 33rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {911},
series = {SIGIR '10}
}

@inproceedings{carmel_qpp_sigir06,
author = {Carmel, David and Yom-Tov, Elad and Darlow, Adam and Pelleg, Dan},
title = {What Makes a Query Difficult?},
year = {2006},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 29th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {390–397},
series = {SIGIR '06}
}

@inproceedings{croft_qpp_sigir02,
author = {Cronen-Townsend, Steve and Zhou, Yun and Croft, W. Bruce},
title = {Predicting Query Performance},
year = {2002},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 25th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {299–306},
series = {SIGIR '02}
}

@inproceedings{cummins_qppSD_sigir11,
author = {Cummins, Ronan and Jose, Joemon and O'Riordan, Colm},
title = {Improved Query Performance Prediction Using Standard Deviation},
year = {2011},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 34th International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {1089–1090},
series = {SIGIR '11}
}

@inproceedings{fernando_correlation_sigir07,
author = {Diaz, Fernando},
title = {Performance Prediction Using Spatial Autocorrelation},
year = {2007},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 30th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {583–590},
series = {SIGIR '07}
}

@inproceedings{qpp_microblog_IPM,
author = {Hasanain, Maram and Malhas, Rana and Elsayed, Tamer},
title = {Query Performance Prediction for Microblog Search: A Preliminary Study},
year = {2014},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the First International Workshop on Social Media Retrieval and Analysis},
pages = {1–6},
series = {SoMeRA '14}
}

@InProceedings{qpp_coherence,
author="He, Jiyin
and Larson, Martha
and de Rijke, Maarten",
editor="Macdonald, Craig
and Ounis, Iadh
and Plachouras, Vassilis
and Ruthven, Ian
and White, Ryen W.",
title="Using Coherence-Based Measures to Predict Query Difficulty",
booktitle="Advances in Information Retrieval",
year="2008",
publisher="Springer Berlin Heidelberg",
pages="689--694",
}

@inproceedings{mothe_linguistics,
  title={Linguistic features to predict query difficulty - a case study on previous TREC campaigns},
  author={J. Mothe and L. Tanguy},
  year={2005}
}

@INPROCEEDINGS{MM_qe_qpp,  
author={D. {Pal} and M. {Mitra} and S. {Bhattacharya}},  
booktitle={2014 Fourth International Conference of Emerging Applications of Information Technology},   
title={Using Multiple Query Expansion Algorithms to Predict Query Performance},   
year={2014},  
pages={361-364},
}

@inproceedings{kurland_sigir14,
author = {Raiber, Fiana and Kurland, Oren},
title = {Query-Performance Prediction: Setting the Expectations Straight},
year = {2014},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 37th International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {13–22},
series = {SIGIR '14}
}

@inproceedings{qpp_ref_list_sigir17,
author = {Roitman, Haggai},
title = {An Enhanced Approach to Query Performance Prediction Using Reference Lists},
year = {2017},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 37th International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {869–872},
series = {Proc. {SIGIR '17}}
}

@inproceedings{qpp_robust_SD_ictir17,
author = {Roitman, Haggai and Erera, Shai and Weiner, Bar},
title = {Robust Standard Deviation Estimation for Query Performance Prediction},
year = {2017},
booktitle = {Proceedings of the ACM SIGIR International Conference on Theory of Information Retrieval},
pages = {245–248},
series = {ICTIR '17}
}

@inproceedings{qpp_dist_IR_sigir05,
author = {Yom-Tov, Elad and Fine, Shai and Carmel, David and Darlow, Adam},
title = {Learning to Estimate Query Difficulty: Including Applications to Missing Content Detection and Distributed Information Retrieval},
year = {2005},
publisher = {ACM},
address = {New York, NY, USA},
pages = {512–519},
series = {SIGIR '05}
}

@inproceedings{qpp_croft_cikm06,
author = {Zhou, Yun and Croft, W. Bruce},
title = {Ranking Robustness: A Novel Framework to Predict Query Performance},
year = {2006},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 15th ACM International Conference on Information and Knowledge Management},
pages = {567–574},
series = {CIKM '06}
}

@inproceedings{carmel_qpp_sigir05,
author = {Yom-Tov, Elad and Fine, Shai and Carmel, David and Darlow, Adam},
title = {Learning to Estimate Query Difficulty: Including Applications to Missing Content Detection and Distributed Information Retrieval},
year = {2005},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 28th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {512–519},
series = {SIGIR '05}
}


% 
% pre-retrieval
% 


@InProceedings{qpp_preret_springer,
author="He, Ben
and Ounis, Iadh",
title="Inferring Query Performance Using Pre-retrieval Predictors",
booktitle="String Processing and Information Retrieval",
year="2004",
pages="43--54",
}

@inproceedings{qpp_preret_ecir08,
author = {Zhao, Ying and Scholer, Falk and Tsegay, Yohannes},
title = {Effective Pre-Retrieval Query Performance Prediction Using Similarity and Variability Evidence},
year = {2008},
publisher = {Springer-Verlag},
pages = {52–64},
series = {ECIR'08}
}

@inproceedings{carmel_sigir10,
author = {Carmel, David and Yom-Tov, Elad},
title = {Estimating the Query Difficulty for Information Retrieval},
year = {2010},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 33rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {911},
numpages = {1},
series = {SIGIR '10}
}

@article{precision_prediction,
author = {Cronen-Townsend, Steve and Zhou, Yun and Croft, W. Bruce},
title = {Precision Prediction Based on Ranked List Coherence},
year = {2006},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {9},
number = {6},
journal = {Inf. Retr.},
month = dec,
pages = {723–755},
numpages = {33},
}

@inproceedings{qpp_using_sd,
author = {Cummins, Ronan and Jose, Joemon and O'Riordan, Colm},
title = {Improved Query Performance Prediction Using Standard Deviation},
year = {2011},
publisher = {ACM},
booktitle = {Proceedings of the 34th International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {1089–1090},
numpages = {2},
series = {SIGIR '11}
}

@inproceedings{survey_preret_qpp,
author = {Hauff, Claudia and Hiemstra, Djoerd and de Jong, Franciska},
title = {A Survey of Pre-Retrieval Query Performance Predictors},
year = {2008},
publisher = {ACM},
booktitle = {Proceedings of the 17th ACM Conference on Information and Knowledge Management},
pages = {1419–1420},
numpages = {2},
series = {CIKM '08}
}

@inproceedings{postret_ictir11,
author = {Kurland, Oren and Shtok, Anna and Carmel, David and Hummel, Shay},
title = {A Unified Framework for Post-Retrieval Query-Performance Prediction},
year = {2011},
booktitle = {Proceedings of the Third International Conference on Advances in Information Retrieval Theory},
pages = {15–26},
numpages = {12},
series = {ICTIR'11}
}

@inproceedings{preret_adcs17,
author = {Thomas, Paul and Scholer, Falk and Bailey, Peter and Moffat, Alistair},
title = {Tasks, Queries, and Rankers in Pre-Retrieval Performance Prediction},
year = {2017},
publisher = {ACM},
booktitle = {Proceedings of the 22nd Australasian Document Computing Symposium},
articleno = {11},
numpages = {4},
series = {ADCS 2017}
}

@article{qpp_ref_2016,
author = {Shtok, Anna and Kurland, Oren and Carmel, David},
title = {Query Performance Prediction Using Reference Lists},
year = {2016},
issue_date = {September 2016},
publisher = {ACM},
address = {New York, NY, USA},
volume = {34},
number = {4},
articleno = {19},
numpages = {34},
}

@MISC{Okapi,
    author = {S.E. Robertson and S. Walker and M.M. Beaulieu and M. Gatford and A. Payne},
    title = {Okapi at TREC-4},
    year = {1996}
}

@article{uef_effect_1977,
author = {Robertson S.E.},
volume = {33},
number = {4},
year = {1977},
title = {The Probability Ranking Principle in IR},
publisher = {MCB UP Ltd},
booktitle = {Journal of Documentation}
}

@InProceedings{pmlr-v15-glorot11a,
  title = 	 {Deep Sparse Rectifier Neural Networks},
  author = 	 {Xavier Glorot and Antoine Bordes and Yoshua Bengio},
  booktitle = 	 {Proceedings of the Fourteenth International Conference on Artificial Intelligence and Statistics},
  pages = 	 {315--323},
  year = 	 {2011},
  volume = 	 {15},
  month = 	 {11--13 Apr},
  abstract = 	 {While logistic sigmoid neurons are more biologically plausible than hyperbolic tangent neurons, the latter work better for training multi-layer neural networks. This paper shows that rectifying neurons are an even better model of biological neurons and yield equal or better performance than hyperbolic tangent networks in spite of the hard non-linearity and non-differentiability at zero, creating sparse representations with true zeros which seem remarkably suitable for naturally sparse data. Even though they can take advantage of semi-supervised setups with extra-unlabeled data, deep rectifier networks can reach their best performance without requiring any unsupervised pre-training on purely supervised tasks with large labeled datasets. Hence, these results can be seen as a new milestone in the attempts at understanding the difficulty in training deep but purely supervised neural networks, and closing the performance gap between neural networks learnt with and without unsupervised pre-training.}
}


@inbook{quantum_neural,
author = {Jiang, Yongyu and Zhang, Peng and Gao, Hui and Song, Dawei},
title = {A Quantum Interference Inspired Neural Matching Model for Ad-Hoc Retrieval},
year = {2020},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {19–28},
}

@inproceedings{akkalyoncu-yilmaz-etal-2019-applying,
    title = "Applying {BERT} to Document Retrieval with Birch",
    author = "Akkalyoncu Yilmaz, Zeynep  and
      Wang, Shengjin  and
      Yang, Wei  and
      Zhang, Haotian  and
      Lin, Jimmy",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP): System Demonstrations",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    pages = "19--24",
}

@inproceedings{drmm_croft,
author = {Guo, Jiafeng and Fan, Yixing and Ai, Qingyao and Croft, W. Bruce},
title = {A Deep Relevance Matching Model for Ad-Hoc Retrieval},
year = {2016},
publisher = {ACM},
booktitle = {Proceedings of the 25th ACM International on Conference on Information and Knowledge Management},
pages = {55–64},
series = {CIKM '16}
}

@inproceedings{knrm_SIGIR17,
author = {Xiong, Chenyan and Dai, Zhuyun and Callan, Jamie and Liu, Zhiyuan and Power, Russell},
title = {End-to-End Neural Ad-Hoc Ranking with Kernel Pooling},
year = {2017},
publisher = {ACM},
booktitle = {Proceedings of the 40th International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {55–64},
series = {SIGIR '17}
}

@inproceedings{conv_knrm,
author = {Dai, Zhuyun and Xiong, Chenyan and Callan, Jamie and Liu, Zhiyuan},
title = {Convolutional Neural Networks for Soft-Matching N-Grams in Ad-Hoc Search},
year = {2018},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the Eleventh ACM International Conference on Web Search and Data Mining},
pages = {126–134},
series = {WSDM '18}
}

@inproceedings{DBLP:conf/sigir/DehghaniZSKC17,
  author    = {Mostafa Dehghani and
               Hamed Zamani and
               Aliaksei Severyn and
               Jaap Kamps and
               W. Bruce Croft},
  title     = {Neural Ranking Models with Weak Supervision},
  booktitle = {{SIGIR}},
  pages     = {65--74},
  publisher = {{ACM}},
  year      = {2017}
}

@inbook{colbert_sigir20,
author = {Khattab, Omar and Zaharia, Matei},
title = {ColBERT: Efficient and Effective Passage Search via Contextualized Late Interaction over BERT},
year = {2020},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {39–48},
}

@inbook{doc_rank_bert_sigir20,
author = {Zhan, Jingtao and Mao, Jiaxin and Liu, Yiqun and Zhang, Min and Ma, Shaoping},
title = {An Analysis of BERT in Document Ranking},
year = {2020},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {1941–1944},
}

@inbook{feature_neural_model_sigir20,
author = {Zhuang, Honglei and Wang, Xuanhui and Bendersky, Michael and Najork, Marc},
title = {Feature Transformation for Neural Ranking Models},
year = {2020},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {1649–1652},
}


@inproceedings{beamsearch,
author = {Zhou, Rong and Hansen, Eric A.},
title = {Beam-Stack Search: Integrating Backtracking with Beam Search},
year = {2005},
isbn = {1577352203},
publisher = {AAAI Press},
booktitle = {Proceedings of the Fifteenth International Conference on International Conference on Automated Planning and Scheduling},
pages = {90–98},
numpages = {9},
location = {Monterey, California, USA},
series = {ICAPS'05}
}

@inproceedings{sigir20_global_emb,
author = {Wang, Ziyang and Wei, Wei and Cong, Gao and Li, Xiao-Li and Mao, Xian-Ling and Qiu, Minghui},
title = {Global Context Enhanced Graph Neural Networks for Session-Based Recommendation},
year = {2020},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {169–178},
numpages = {10},
location = {Virtual Event, China},
series = {SIGIR '20}
}

@inproceedings{encoding_history,
author = {Zhou, Yujia and Dou, Zhicheng and Wen, Ji-Rong},
title = {Encoding History with Context-Aware Representation Learning for Personalized Search},
year = {2020},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {1111–1120},
numpages = {10},
location = {Virtual Event, China},
series = {SIGIR '20}
}

@inproceedings{personalized_wordemb,
author = {Yao, Jing and Dou, Zhicheng and Wen, Ji-Rong},
title = {Employing Personal Word Embeddings for Personalized Search},
year = {2020},
publisher = {ACM},
address = {New York, NY, USA},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {1359–1368},
numpages = {10},
location = {Virtual Event, China},
series = {SIGIR '20}
}

@inproceedings{hred_attention,
  author    = {Wanyu Chen and
               Fei Cai and
               Honghui Chen and
               Maarten de Rijke},
  title     = {Attention-based Hierarchical Neural Query Suggestion},
  booktitle = {{SIGIR}},
  pages     = {1093--1096},
  publisher = {{ACM}},
  year      = {2018}
}

@inproceedings{TRECCS_ltr,
  author    = {Dominic Seyler and
               Praveen Chandar and
               Matthew Davis},
  title     = {An Information Retrieval Framework for Contextual Suggestion Based
               on Heterogeneous Information Network Embeddings},
  booktitle = {{SIGIR}},
  pages     = {953--956},
  publisher = {{ACM}},
  year      = {2018}
}

@inproceedings{serpsize,
  author    = {Diane Kelly and
               Leif Azzopardi},
  title     = {How many results per page?: {A} Study of {SERP} Size, Search Behavior
               and User Experience},
  booktitle = {{SIGIR}},
  pages     = {183--192},
  publisher = {{ACM}},
  year      = {2015}
}

@inproceedings{querysuggestion,
  author    = {Wasi Uddin Ahmad and
               Kai{-}Wei Chang and
               Hongning Wang},
  title     = {Context Attentive Document Ranking and Query Suggestion},
  booktitle = {{SIGIR}},
  pages     = {385--394},
  publisher = {{ACM}},
  year      = {2019}
}

@inproceedings{usersat1,
  author    = {Jiqun Liu and
               Fangyuan Han},
  title     = {Investigating Reference Dependence Effects on User Search Interaction
               and Satisfaction: {A} Behavioral Economics Perspective},
  booktitle = {{SIGIR}},
  pages     = {1141--1150},
  publisher = {{ACM}},
  year      = {2020}
}

@inproceedings{usersat2,
  author    = {Hamed Zamani and
               Bhaskar Mitra and
               Everest Chen and
               Gord Lueck and
               Fernando Diaz and
               Paul N. Bennett and
               Nick Craswell and
               Susan T. Dumais},
  title     = {Analyzing and Learning from User Interactions for Search Clarification},
  booktitle = {{SIGIR}},
  pages     = {1181--1190},
  publisher = {{ACM}},
  year      = {2020}
}

@inproceedings{usersat3,
  author    = {Azin Ashkan and
               Donald Metzler},
  title     = {Revisiting Online Personal Search Metrics with the User in Mind},
  booktitle = {{SIGIR}},
  pages     = {625--634},
  publisher = {{ACM}},
  year      = {2019}
}

@inproceedings{usersat4,
  author    = {Matthew Mitsui and
               Chirag Shah},
  title     = {Bridging Gaps: Predicting User and Task Characteristics from Partial
               User Information},
  booktitle = {{SIGIR}},
  pages     = {415--424},
  publisher = {{ACM}},
  year      = {2019}
}

@inproceedings{DNN-Graph,
author = {Cao, Shaosheng and Lu, Wei and Xu, Qiongkai},
title = {Deep Neural Networks for Learning Graph Representations},
year = {2016},
publisher = {AAAI Press},
booktitle = {Proceedings of the Thirtieth AAAI Conference on Artificial Intelligence},
pages = {1145–1152},
numpages = {8},
location = {Phoenix, Arizona},
series = {AAAI’16}
}

@inproceedings{graph-autoenc2,
author = {Pan, Shirui and Hu, Ruiqi and Long, Guodong and Jiang, Jing and Yao, Lina and Zhang, Chengqi},
title = {Adversarially Regularized Graph Autoencoder for Graph Embedding},
year = {2018},
isbn = {9780999241127},
publisher = {AAAI Press},
booktitle = {Proceedings of the 27th International Joint Conference on Artificial Intelligence},
pages = {2609–2615},
series = {IJCAI’18}
}
  

@inproceedings{graph-autoenc,
  author    = {Tengfei Ma and
               Jie Chen and
               Cao Xiao},
  title     = {Constrained Generation of Semantically Valid Graphs via Regularizing
               Variational Autoencoders},
  booktitle = {NeurIPS},
  pages     = {7113--7124},
  year      = {2018}
}

@InProceedings{pmlr-v80-bojchevski18a,
  title = 	 {{N}et{GAN}: Generating Graphs via Random Walks},
  author = 	 {Aleksandar Bojchevski and Oleksandr Shchur and Daniel Zügner and Stephan Günnemann},
  booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
  pages = 	 {610--619},
  year = 	 {2018},
  editor = 	 {Jennifer Dy and Andreas Krause},
  volume = 	 {80},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {10--15 Jul},
  publisher = 	 {PMLR}
}  

@inproceedings{deepwalk,
  author    = {Bryan Perozzi and
               Rami Al{-}Rfou and
               Steven Skiena},
  title     = {DeepWalk: online learning of social representations},
  booktitle = {{KDD'14}},
  pages     = {701--710},
  year      = {2014}
}

@inproceedings{devlin-etal-2019-bert,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
    booktitle = {Proc. of {NAACL'19}},
    year = "2019",
    pages = "4171--4186",
}

@inproceedings{birch,
  author    = {Zeynep Akkalyoncu Yilmaz and
               Shengjin Wang and
               Wei Yang and
               Haotian Zhang and
               Jimmy Lin},
  title     = {Applying {BERT} to Document Retrieval with Birch},
  pages     = {19--24},
  year      = {2019},
}

@inproceedings{drmm,
author = {Guo, Jiafeng and Fan, Yixing and Ai, Qingyao and Croft, W. Bruce},
title = {A Deep Relevance Matching Model for Ad-Hoc Retrieval},
booktitle = {Proc. of CIKM'16},
pages = {55–64},
year={2016}
}

@inproceedings{convnet-search,
  author    = {Jinfeng Rao and
               Wei Yang and
               Yuhao Zhang and
               Ferhan T{\"{u}}re and
               Jimmy Lin},
  title     = {Multi-Perspective Relevance Matching with Hierarchical ConvNets for
               Social Media Search},
  booktitle = {{AAAI}},
  pages     = {232--240},
  publisher = {{AAAI} Press},
  year      = {2019}
}

@misc{smartstoplist,
  title = {{SMART} stopword list},
  howpublished = {\url{https://www.lextek.com/manuals/onix/stopwords2.html},},
  year = {2019}, 
}

@article{Koskela:2018,
 author = {Koskela, Markus and Luukkonen, Petri and Ruotsalo, Tuukka and Sj\"{O}berg, Mats and Flor{\'e}en, Patrik},
 title = {Proactive Information Retrieval by Capturing Search Intent from Primary Task Context},
 journal = {ACM Trans. Interact. Intell. Syst.},
 year = {2018},
 pages = {20:1--20:25},
 } 

@inproceedings{NMF_ProbabilisticMatrixFactorization,
 author = {Salakhutdinov, Ruslan and Mnih, Andriy},
 title = {Bayesian Probabilistic Matrix Factorization Using Markov Chain Monte Carlo},
 booktitle = {Proc. of ICML 2008},
 pages = {880--887},
}
@inproceedings{Kanoulas:2011,
 author = {Kanoulas, Evangelos and Carterette, Ben and Clough, Paul D. and Sanderson, Mark},
 title = {Evaluating Multi-query Sessions},
 booktitle = {Proc. SIGIR 2011},
 pages = {1053--1062},
} 


@INPROCEEDINGS{Fox94combinationof,
    author = {Joseph A. Shaw and Edward A. Fox and Joseph A. Shaw and Edward A. Fox},
    title = {Combination of Multiple Searches},
    booktitle = {Proc. of TREC-2 1994},
    pages = {243--252}
}

@inproceedings{Ponte:1998,
 author = {Ponte, Jay M. and Croft, W. Bruce},
 title = {A Language Modeling Approach to Information Retrieval},
 booktitle = {Proc. of SIGIR 1998},
 year = {1998},
 pages = {275--281}
} 
@inproceedings{Puolamaki,
 author = {Puolam\"{a}ki, Kai and Saloj\"{a}rvi, Jarkko and Savia, Eerika and Simola, Jaana and Kaski, Samuel},
 title = {Combining Eye Movements and Collaborative Filtering for Proactive Information Retrieval},
 booktitle = {Proceedings of SIGIR 2005},
 pages = {146--153},
 year={2005}
 } 
 
 @inproceedings{Vuong:2017,
 author = {Vuong, Tung and Jacucci, Giulio and Ruotsalo, Tuukka},
 title = {Proactive Information Retrieval via Screen Surveillance},
 booktitle = {Proceedings of SIGIR 2017},
 pages = {1313--1316},
 year={2017}
 } 
 @inproceedings{Fitchett:2012,
 author = {Fitchett, Stephen and Cockburn, Andy},
 title = {AccessRank: Predicting What Users Will Do Next},
 booktitle = {Proceedings of the SIGCHI},
 year={2012},
  pages = {2239--2242},
 }
  @inproceedings{Tran:2016,
 author = {Tran, Tuan A. and Schwarz, Sven and Nieder{\'e}e, Claudia and Maus, Heiko and Kanhabua, Nattiya},
 title = {The Forgotten Needle in My Collections: Task-Aware Ranking of Documents in Semantic Information Space},
 booktitle = {Proceedings of CHIIR},
 year={2016},
 pages = {13--22}
 }
 @article{Dumais:2016,
 author = {Dumais, Susan and Cutrell, Edward and Cadiz, J. J. and Jancke, Gavin and Sarin, Raman and Robbins, Daniel C.},
 title = {Stuff I'Ve Seen: A System for Personal Information Retrieval and Re-Use},
 journal = {SIGIR Forum},
 pages = {28--35},
 year={2016}
 }
 @inproceedings{Dumais:2004,
 author = {Dumais, Susan and Cutrell, Edward and Sarin, Raman and Horvitz, Eric},
 title = {Implicit Queries (IQ) for Contextualized Search},
 booktitle = {Proceedings of SIGIR},
 year={2004},
 pages = {594--594}
 } 

@article{Cormack:2011,
 author = {Cormack, Gordon V. and Smucker, Mark D. and Clarke, Charles L.},
 title = {Efficient and Effective Spam Filtering and Re-ranking for Large Web Datasets},
 volume = {14},
 number = {5},
 journal = {Inf. Retr.},
 year = {2011},
 pages = {441--465}
} 

@inproceedings{RoyGMJ16,
  author    = {Dwaipayan Roy and
               Debasis Ganguly and
               Mandar Mitra and
               Gareth J. F. Jones},
  title     = {Word Vector Compositionality based Relevance Feedback using Kernel
               Density Estimation},
  booktitle = {Proc. of CIKM 2016},
  pages     = {1281--1290},
  year = {2016}
}

@inproceedings{HassanAwadallah,
 author = {Hassan Awadallah, Ahmed and White, Ryen W. and Pantel, Patrick and Dumais, Susan T. and Wang, Yi-Min},
 title = {Supporting Complex Search Tasks},
 booktitle = {Proc. of CIKM 2014},
 pages = {829--838},
 year={2014}
}

@inproceedings{Lavrenko2001,
 author = {Lavrenko, Victor and Croft, W. Bruce},
 title = {Relevance Based Language Models},
 booktitle = {Proc. of SIGIR  2001},
 pages = {120--127},
 year={2001}
 } 


@inproceedings{Wang:2013,
 author = {Wang, Hongning and Song, Yang and Chang, Ming-Wei and He, Xiaodong and White, Ryen W. and Chu, Wei},
 title = {Learning to Extract Cross-session Search Tasks},
  publisher = {ACM},
 booktitle = {Proc. of WWW 2013},
 pages = {1353--1364},
 }
@inproceedings{Kong:2015,
 author = {Kong, Weize and Li, Rui and Luo, Jie and Zhang, Aston and Chang, Yi and Allan, James},
 title = {Predicting Search Intent Based on Pre-Search Context},
 booktitle = {Proc. of SIGIR 2015},
 pages = {503--512}
}
@inproceedings{Sordoni:2015,
 author = {Sordoni, Alessandro and Bengio, Yoshua and Vahabi, Hossein and Lioma, Christina and Grue Simonsen, Jakob and Nie, Jian-Yun},
 title = {A Hierarchical Recurrent Encoder-Decoder for Generative Context-Aware Query Suggestion},
 booktitle = {Proc. of CIKM 2015},
 pages = {553--562},
  } 
 @inproceedings{Jones,
 author = {Jones, Rosie and Klinkner, Kristina Lisa},
 title={Beyond the Session Timeout: Automatic Hierarchical
Segmentation of Search Topics in Query Logs},
 booktitle = {Proc. of CIKM '08},
 pages = {699--708}
 } 
 
@inproceedings{Boldi,
 author = {Boldi, Paolo and Bonchi, Francesco and Castillo, Carlos and Donato, Debora and Gionis, Aristides and Vigna, Sebastiano},
 title = {The Query-flow Graph: Model and Applications},
 booktitle = {Proc. of CIKM 2008},
 pages = {609--618},
 year={2008}
}

@inproceedings{Mehrotra:2017,
 author = {Mehrotra, Rishabh and Yilmaz, Emine},
 title = {Task Embeddings: Learning Query Embeddings Using Task Context},
 booktitle = {Proc. of CIKM 2017},
 pages = {2199--2202},
 } 
@inproceedings{MehrotraY17,
  author    = {Rishabh Mehrotra and
               Emine Yilmaz},
  title     = {Extracting Hierarchies of Search Tasks {\&} Subtasks via a Bayesian Nonparametric Approach},
  booktitle = {Proc. of SIGIR 2017},
  pages     = {285--294},
 }

@inproceedings{RhaSB17,
  author    = {Eun Youp Rha and
               Wei Shi and
               Nicholas J. Belkin},
  title     = {An exploration of reasons for query reformulations},
  booktitle = {In Proc. of {ASIST}'17},
  pages     = {337--346},
  year      = {2017}
}

@article{LiuLB16,
  author    = {Jingjing Liu and
               Chang Liu and
               Nicholas J. Belkin},
  title     = {Predicting information searchers' topic knowledge at different search
               stages},
  journal   = {{JASIST}},
  year = {2016},
  pages     = {2652--2666},
  }

@inproceedings{CarteretteKHC14,
  author    = {Ben Carterette and
               Evangelos Kanoulas and
               Mark M. Hall and
               Paul D. Clough},
  title     = {Overview of the {TREC} 2014 Session Track},
  booktitle = {Proc. of TREC 2014},
  year={2014}
 }

@inproceedings{Feild,
 author = {Feild, Henry and Allan, James},
 title = {Task-aware Query Recommendation},
 booktitle = {Proc. of SIGIR 2013},
 pages = {83--92},
 year={2013}
 }
 
@inproceedings{Levine,
 author = {Levine, Nir and Roitman, Haggai and Cohen, Doron},
 title = {An Extended Relevance Model for Session Search},
 booktitle = {Proc. of SIGIR 2017},
 pages = {865--868}
} 
@inproceedings{Zhang,
 author = {Zhang, Sicong and Guan, Dongyi and Yang, Hui},
 title = {Query Change As Relevance Feedback in Session Search},
 booktitle = {Proc. of SIGIR 2013},
 pages = {821--824},
} 
@inproceedings{Li,
 author = {Li, Guoliang and Wang, Jiannan and Li, Chen and Feng, Jianhua},
 title = {Supporting Efficient Top-k Queries in Type-ahead Search},
 booktitle = {Proc. of SIGIR 2012},
  pages = {355--364}
} 
@inproceedings{Kato,
 author = {Kato, Makoto P. and Yamamoto, Takehiro and Ohshima, Hiroaki and Tanaka, Katsumi},
 title = {Investigating Users' Query Formulations for Cognitive Search Intents},
 booktitle = {Proc. of SIGIR 2013},
 pages = {577--586},
 
} 
@inproceedings{Tan,
 author = {Tan, Bin and Shen, Xuehua and Zhai, ChengXiang},
 title = {Mining Long-term Search History to Improve Search Accuracy},
 booktitle = {Proc. of SIGKDD 2006},
 pages = {718--723},
 }
@inproceedings{Qvarfordt,
 author = {Qvarfordt, Pernilla and Golovchinsky, Gene and Dunnigan, Tony and Agapie, Elena},
 title = {Looking Ahead: Query Preview in Exploratory Search},
 booktitle = {Proc. of SIGIR 2013},
 pages = {243--252},
}

@inproceedings{Mikolov13,
  author    = {Tomas Mikolov and
               Ilya Sutskever and
               Kai Chen and
               Gregory S. Corrado and
               Jeffrey Dean},
  title     = {Distributed Representations of Words and Phrases and their Compositionality},
  booktitle = {Proceedings of NIPS 2013},
  pages     = {3111--3119},
 }
 
@inproceedings{sen123,
  author    = {Procheta Sen and
               Debasis Ganguly and
               Gareth J.F. Jones},
  title     = {Tempo-Lexical Context driven Word Embedding for Cross-Session Search Task Extraction},
  booktitle = {Proc of {NAACL-HLT} 2018},
  pages = "283--292",
  } 
 
 @inproceedings{Peters:2018,
  author={Peters, Matthew E. and  Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  title={Deep contextualized word representations},
  booktitle={Proc. of NAACL 2018},
  pages = "2227--2237",
  }


@inproceedings{Sen:2018,
 author = {Sen, Procheta and Ganguly, Debasis and Jones, Gareth},
 title = {Procrastination is the Thief of Time: Evaluating the Effectiveness of Proactive Search Systems},
 booktitle = {Proc. of SIGIR 2018},
 pages = {1157--1160},
 } 

@inproceedings{Grover:2016,
 author = {Grover, Aditya and Leskovec, Jure},
 title = {Node2Vec: Scalable Feature Learning for Networks},
 booktitle = {Proc. of ACM SIGKDD'16},
 pages = {855--864},
 year={2016}
} 

@inproceedings{Li:2012,
 author = {Li, Ruirui and Kao, Ben and Bi, Bin and Cheng, Reynold and Lo, Eric},
 title = {DQR: A Probabilistic Approach to Diversified Query Recommendation},
 booktitle = {Proc. of CIKM 2012},
 year={2012},
 pages = {16--25}
 } 
 @inproceedings{Mitra:2014,
 author = {Mitra, Bhaskar and Shokouhi, Milad and Radlinski, Filip and Hofmann, Katja},
 title = {On User Interactions with Query Auto-completion},
 booktitle = {Proceedings of the 37th International ACM SIGIR Conference on Research Development in Information Retrieval},
 year = {2014},
 pages = {1055--1058}
 } 
@inproceedings{Muntean:2013,
 author = {Muntean, Cristina Ioana and Nardini, Franco Maria and Silvestri, Fabrizio and Sydow, Marcin},
 title = {Learning to Shorten Query Sessions},
 booktitle = {Proc. of WWW 2013},
 year={2013},
 pages = {131--132},
 } 
 @article{Lucchese,
 author = {Lucchese, Claudio and Orlando, Salvatore and Perego, Raffaele and Silvestri, Fabrizio and Tolomei, Gabriele},
 title = {Discovering Tasks from Search Engine Query Logs},
 journal = {ACM Transactions Inf. Syst.},
 year = {2013},
 pages = {14:1--14:43},
 } 
 @inproceedings{Bonchi:2012,
 author = {Bonchi, Francesco and Perego, Raffaele and Silvestri, Fabrizio and Vahabi, Hossein and Venturini, Rossano},
 title = {Efficient Query Recommendations in the Long Tail via Center-piece Subgraphs},
 publisher={ACM},
 booktitle = {Proc. of SIGIR 2012},
 pages = {345--354},
 } 
@inproceedings{Le:2014,
 author = {Le, Quoc and Mikolov, Tomas},
 title = {Distributed Representations of Sentences and Documents},
 booktitle = {Proc. of ICML 2014},
 pages = {II-1188--II-1196}
} 

@inproceedings{Zamani:2017,
 author = {Zamani, Hamed and Croft, W. Bruce},
 title = {Relevance-based Word Embedding},
 booktitle = {Proc. of SIGIR 2017},
 pages = {505--514},
address = {New York, NY, USA},
 } 
 
 @inproceedings{Dehghani:2017,
 author = {Dehghani, Mostafa and Zamani, Hamed and Severyn, Aliaksei and Kamps, Jaap and Croft, W. Bruce},
 title = {Neural Ranking Models with Weak Supervision},
 booktitle = {Proc. of {SIGIR 2017}},
  pages = {65--74},
} 

@inproceedings{Wang:2016,
 author = {Wang, Suhang and Tang, Jiliang and Aggarwal, Charu and Liu, Huan},
 title = {Linked Document Embedding for Classification},
 booktitle = {Proc. of CIKM 2016},
 pages = {115--124},
 } 
 
@ARTICLE{gcnnsurvey,
author={Z. {Wu} and S. {Pan} and F. {Chen} and G. {Long} and C. {Zhang} and P. S. {Yu}},
journal={IEEE Transactions on Neural Networks and Learning Systems}, 
title={A Comprehensive Survey on Graph Neural Networks}, 
year={2020},
pages={1-21},
}

@inproceedings{node2vec_attention,
title = {Watch Your Step: Learning Node Embeddings via Graph Attention},
author = {Abu-El-Haija, Sami and Perozzi, Bryan and Al-Rfou, Rami and Alemi, Alexander A},
booktitle = {Advances in Neural Information Processing Systems 31},
pages = {9180--9190},
year = {2018}
}

@article{node2vec_survey,
  author    = {Peng Cui and
               Xiao Wang and
               Jian Pei and
               Wenwu Zhu},
  title     = {A Survey on Network Embedding},
  journal   = {{IEEE} Trans. Knowl. Data Eng.},
  volume    = {31},
  number    = {5},
  pages     = {833--852},
  year      = {2019}
}

@inproceedings{graphconv,
author = {Wu, Le and Yang, Yonghui and Zhang, Kun and Hong, Richang and Fu, Yanjie and Wang, Meng},
title = {Joint Item Recommendation and Attribute Inference: An Adaptive Graph Convolutional Network Approach},
year = {2020},
booktitle = {Proc. of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {679–688},}

@inproceedings{attention,
author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, undefinedukasz and Polosukhin, Illia},
title = {Attention is All You Need},
booktitle = {Proceedings of the 31st International Conference on Neural Information Processing Systems},
pages = {6000–6010},
}

@inproceedings{NasreenJaleel_RM3,
  author    = {Nasreen Abdul Jaleel and
               James Allan and
               W. Bruce Croft and
               Fernando Diaz and
               Leah S. Larkey and
               Xiaoyan Li and
               Mark D. Smucker and
               Courtney Wade},
  title     = {UMass at {TREC} 2004: Novelty and {HARD}},
  booktitle = {TREC 2004},
  year = {2004},
}

@book{linear_regression_book,
author = {Yan, Xin and Su, Xiao Gang},
title = {Linear Regression Analysis: Theory and Computing},
year = {2009},
isbn = {9789812834102},
publisher = {World Scientific Publishing Co., Inc.},
address = {USA},
}

@inproceedings{uqvdataset,
author = {Bailey, Peter and Moffat, Alistair and Scholer, Falk and Thomas, Paul},
title = {UQV100: A Test Collection with Query Variability},
booktitle = {In Proc. of {SIGIR '16}},
year = {2016},
pages = {725–728},
}

@inproceedings{uqvconsistency,
author = {Bailey, Peter and Moffat, Alistair and Scholer, Falk and Thomas, Paul},
title = {Retrieval Consistency in the Presence of Query Variations},
year = {2017},
booktitle = {Proc. of {SIGIR '17}},
pages = {395–404},
}
  
@inproceedings{lmdir,
author = {Zhai, Chengxiang and Lafferty, John},
title = {A Study of Smoothing Methods for Language Models Applied to Ad Hoc Information Retrieval},
year = {2001},
booktitle = {Proceedings of the 24th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {334–342},
series = {SIGIR '01}
}

@inproceedings{query_variants_kurland,
  author    = {Oleg Zendel and
               Anna Shtok and
               Fiana Raiber and
               Oren Kurland and
               J. Shane Culpepper},
  title     = {Information Needs, Queries, and Query Performance Prediction},
  booktitle = {Proc. of {SIGIR '19}},
  pages     = {395--404},
  year      = {2019}
}

@article{kurland_tois12,
author = {Shtok, Anna and Kurland, Oren and Carmel, David and Raiber, Fiana and Markovits, Gad},
title = {Predicting Query Performance by Query-Drift Estimation},
year = {2012},
publisher = {ACM},
volume = {30},
number = {2},
journal = {ACM Trans. Inf. Syst.},
articleno = {11},
numpages = {35},
}

@inproceedings{zamani_clarifying_sigir,
  author    = {Mohammad Aliannejadi and
               Hamed Zamani and
               Fabio Crestani and
               W. Bruce Croft},
  title     = {Asking Clarifying Questions in Open-Domain Information-Seeking Conversations},
  booktitle = {{SIGIR}},
  pages     = {475--484},
  publisher = {{ACM}},
  year      = {2019}
}

@inproceedings{zamani_clarifying_www,
author = {Zamani, Hamed and Dumais, Susan and Craswell, Nick and Bennett, Paul and Lueck, Gord},
title = {Generating Clarifying Questions for Information Retrieval},
year = {2020},
publisher = {ACM},
booktitle = {Proceedings of The Web Conference 2020},
pages = {418–428},
series = {WWW '20}
}

@inproceedings{croft_sigir07,
author = {Zhou, Yun and Croft, W. Bruce},
title = {Query Performance Prediction in Web Search Environments},
year = {2007},
booktitle = {Proceedings of the 30th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {543–550},
series = {SIGIR '07}
}

@inproceedings{Lavrenko_RLM2001:RBL:383952.383972,
 author = {Lavrenko, Victor and Croft, W. Bruce},
 title = {Relevance Based Language Models},
 booktitle = {Proc. of {SIGIR '01}},
 year = {2001},
 isbn = {1-58113-331-6},
 location = {New Orleans, Louisiana, USA},
 pages = {120--127},
 numpages = {8},
 acmid = {383972},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{hamed_neuralqpp,
author = {Zamani, Hamed and Croft, W. Bruce and Culpepper, J. Shane},
title = {Neural Query Performance Prediction Using Weak Supervision from Multiple Signals},
year = {2018},
publisher = {ACM},
booktitle = {The 41st International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {105–114},
series = {SIGIR '18}
}

@inproceedings{kdrelm_DG,
author = {Roy, Dwaipayan and Ganguly, Debasis and Mitra, Mandar and Jones, Gareth J.F.},
title = {Word Vector Compositionality Based Relevance Feedback Using Kernel Density Estimation},
year = {2016},
publisher = {ACM},
booktitle = {Proceedings of the 25th ACM International on Conference on Information and Knowledge Management},
pages = {1281–1290},
series = {CIKM '16}
}

@inbook{query_variants_DG,
author = {Chakraborty, Anirban and Ganguly, Debasis and Conlan, Owen},
title = {Retrievability Based Document Selection for Relevance Feedback with Automatically Generated Query Variants},
year = {2020},
publisher = {ACM},
booktitle = {Proceedings of the 29th ACM International Conference on Information &amp; Knowledge Management},
pages = {125–134},
}

@inproceedings{factored_rlm_DG,
author = {Chakraborty, Anirban and Ganguly, Debasis and Caputo, Annalina and Lawless, S\'{e}amus},
title = {A Factored Relevance Model for Contextual Point-of-Interest Recommendation},
year = {2019},
publisher = {ACM},
booktitle = {Proceedings of the 2019 ACM SIGIR International Conference on Theory of Information Retrieval},
pages = {157–164},
series = {ICTIR '19}
}

@inbook{recommendation_DG_sigir20,
author = {Chakraborty, Anirban and Ganguly, Debasis and Conlan, Owen},
title = {Relevance Models for Multi-Contextual Appropriateness in Point-of-Interest Recommendation},
year = {2020},
publisher = {ACM},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {1981–1984},
numpages = {4}
}

@inbook{reinforcement_RLM_sigir20,
author = {Montazeralghaem, Ali and Zamani, Hamed and Allan, James},
title = {A Reinforcement Learning Framework for Relevance Feedback},
year = {2020},
publisher = {ACM},
booktitle = {Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {59–68},
}

@article{qpp_DG_IPM,
title = "Estimating Gaussian mixture models in the local neighbourhood of embedded word vectors for query performance prediction",
journal = {{Information Processing and Management}},
volume = "56",
number = "3",
pages = "1026 - 1045",
year = "2019",
author = "Dwaipayan Roy and Debasis Ganguly and Mandar Mitra and Gareth J.F. Jones",
}

@inproceedings{metasearch_SIGIR05,
  title={Metasearch and Federation using Query Difficulty Prediction},
  author={E. Yom-Tov and S. Fine and David Carmel and Adam Darlow},
  year={2005}
}

@inproceedings{matrix_RLM_hamed,
author = {Zamani, Hamed and Dadashkarimi, Javid and Shakery, Azadeh and Croft, W. Bruce},
title = {Pseudo-Relevance Feedback Based on Matrix Factorization},
year = {2016},
booktitle = {Proc. 25th ACM International on Conference on Information and Knowledge Management},
pages = {1483–1492},
series = {CIKM '16}
}

@inproceedings{wig_croft_SIGIR07,
author = {Zhou, Yun and Croft, W. Bruce},
title = {Query Performance Prediction in Web Search Environments},
year = {2007},
booktitle = {Proc. 30th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {543–550},
series = {SIGIR '07}
}

@article{wig_hauff,
author = {Hauff, Claudia},
title = {Predicting the Effectiveness of Queries and Retrieval Systems},
year = {2010},
issue_date = {June 2010},
address = {New York, NY, USA},
volume = {44},
number = {1},
journal = {SIGIR Forum},
month = aug,
pages = {88},
numpages = {1}
}

@inproceedings{uef_kurland_sigir10,
author = {Shtok, Anna and Kurland, Oren and Carmel, David},
title = {Using Statistical Decision Theory and Relevance Models for Query-Performance Prediction},
year = {2010},
booktitle = {Proceedings of the 33rd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {259–266},
series = {SIGIR '10}
}

@inproceedings{croft_cikm04,
author = {Cronen-Townsend, Steve and Zhou, Yun and Croft, W. Bruce},
title = {A Framework for Selective Query Expansion},
year = {2004},
booktitle = {Proceedings of the Thirteenth ACM International Conference on Information and Knowledge Management},
pages = {236–237},
series = {CIKM '04}
}

@article{maxidf_turpin_2004,
author = {Scholer, Falk and Williams, Hugh E. and Turpin, Andrew},
title = {Query Association Surrogates for Web Search: Research Articles},
year = {2004},
issue_date = {May 2004},
publisher = {John Wiley &amp; Sons, Inc.},
address = {USA},
volume = {55},
number = {7},
journal = {J. Am. Soc. Inf. Sci. Technol.},
month = may,
pages = {637–650},
numpages = {14}
}

@inproceedings{web_track_10,
title={Overview of the TREC 2010 Web Track},
author={C. Clarke and Nick Craswell and I. Soboroff and G. Cormack},
booktitle={TREC},
year={2010}
}

% =========== rel works ============

@inproceedings{dr_we_variation,
author = {Roy, Dwaipayan and Ganguly, Debasis and Bhatia, Sumit and Bedathur, Srikanta and Mitra, Mandar},
title = {Using Word Embeddings for Information Retrieval: How Collection and Term Normalization Choices Affect Performance},
year = {2018},
booktitle = {Proceedings of the 27th ACM International Conference on Information and Knowledge Management},
pages = {1835–1838},
series = {CIKM '18}
}

@inproceedings{zobel_cikm09,
author = {Armstrong, Timothy G. and Moffat, Alistair and Webber, William and Zobel, Justin},
title = {Improvements That Don't Add up: Ad-Hoc Retrieval Results since 1998},
year = {2009},
booktitle = {Proceedings of the 18th ACM Conference on Information and Knowledge Management},
pages = {601–610},
series = {CIKM '09}
}

@inproceedings{zobel_sigir98,
author = {Zobel, Justin},
title = {How Reliable Are the Results of Large-Scale Information Retrieval Experiments?},
year = {1998},
booktitle = {Proceedings of the 21st Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {307–314},
numpages = {8},
series = {SIGIR '98}
}

@inproceedings{raiber_sigir14,
author = {Raiber, Fiana and Kurland, Oren},
title = {Query-Performance Prediction: Setting the Expectations Straight},
year = {2014},
booktitle = {Proceedings of the 37th International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {13–22},
numpages = {10},
series = {SIGIR '14}
}

@inproceedings{emine_inferred_ap,
  author    = {Javed A. Aslam and
               Emine Yilmaz},
  title     = {Inferring document relevance from incomplete information},
  booktitle = {Proceedings of the Sixteenth {ACM} Conference on Information and Knowledge Management, {CIKM}},
  pages     = {633--642},
  publisher = {{ACM}},
  year      = {2007},
}

@inproceedings{emine_estimate_ap,
  author    = {Emine Yilmaz and
               Evangelos Kanoulas and
               Javed A. Aslam},
  title     = {A simple and efficient sampling method for estimating {AP} and {NDCG}},
  booktitle = {Proceedings of the 31st Annual International {ACM} {SIGIR} Conference on Research and Development in Information Retrieval, {SIGIR}},
  pages     = {603--610},
  publisher = {{ACM}},
  year      = {2008},
}

@inproceedings{emine_estimate_ap_cikm06,
author = {Yilmaz, Emine and Aslam, Javed A.},
title = {Estimating Average Precision with Incomplete and Imperfect Judgments},
year = {2006},
publisher = {Association for Computing Machinery},
booktitle = {Proceedings of the 15th ACM International Conference on Information and Knowledge Management},
pages = {102–111},
numpages = {10},
series = {CIKM '06}
}

@inproceedings{reproduce_cikm08,
author = {Azzopardi, Leif and Vinay, Vishwa},
title = {Retrievability: An Evaluation Measure for Higher Order Information Access Tasks},
year = {2008},
publisher = {ACM},
booktitle = {Proceedings of the 17th ACM Conference on Information and Knowledge Management},
pages = {561–570},
numpages = {10},
series = {CIKM '08}
}

@inproceedings{buckley_eval_stability,
author = {Buckley, Chris and Voorhees, Ellen M.},
title = {Evaluating Evaluation Measure Stability},
year = {2000},
isbn = {1581132263},
publisher = {Association for Computing Machinery},
booktitle = {Proceedings of the 23rd Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {33–40},
numpages = {8},
series = {SIGIR '00}
}

@inproceedings{buckley_bias_pooling,
  author    = {Chris Buckley and
               Darrin Dimmick and
               Ian Soboroff and
               Ellen M. Voorhees},
  title     = {Bias and the limits of pooling},
  booktitle = {{SIGIR} 2006: Proceedings of the 29th Annual International {ACM} {SIGIR}
               Conference on Research and Development in Information Retrieval, Seattle,
               Washington, USA, August 6-11, 2006},
  pages     = {619--620},
  publisher = {{ACM}},
  year      = {2006},
  biburl    = {https://dblp.org/rec/conf/sigir/BuckleyDSV06.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{buckley_incomplete_info,
  author    = {Chris Buckley and
               Ellen M. Voorhees},
  editor    = {Mark Sanderson and
               Kalervo J{\"{a}}rvelin and
               James Allan and
               Peter Bruza},
  title     = {Retrieval evaluation with incomplete information},
  booktitle = {{SIGIR} 2004: Proceedings of the 27th Annual International {ACM} {SIGIR}
               Conference on Research and Development in Information Retrieval, Sheffield,
               UK, July 25-29, 2004},
  pages     = {25--32},
  publisher = {{ACM}},
  year      = {2004},
  biburl    = {https://dblp.org/rec/conf/sigir/BuckleyV04.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}




@article{carmel2010monograph,
  title={Estimating the query difficulty for information retrieval},
  author={Carmel, David and Yom-Tov, Elad},
  journal={Synthesis Lectures on Information Concepts, Retrieval, and Services},
  volume={2},
  number={1},
  pages={1--89},
  year={2010},
  publisher={Morgan \& Claypool Publishers}
}


@article{neural_hype_sigforum,
author = {Lin, Jimmy},
title = {The Neural Hype, Justified! A Recantation},
year = {2021},
issue_date = {December 2019},
publisher = {Association for Computing Machinery},
volume = {53},
number = {2},
journal = {SIGIR Forum},
pages = {88–93},
numpages = {6}
}

@inproceedings{neural_hype_sigir19,
author = {Yang, Wei and Lu, Kuang and Yang, Peilin and Lin, Jimmy},
title = {Critically Examining the "Neural Hype": Weak Baselines and the Additivity of Effectiveness Gains from Neural Ranking Models},
year = {2019},
publisher = {Association for Computing Machinery},
booktitle = {Proceedings of the 42nd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {1129–1132},
numpages = {4},
series = {SIGIR'19}
}

@inproceedings{scholer09,
author = {Scholer, Falk and Garcia, Steven},
title = {A Case for Improved Evaluation of Query Difficulty Prediction},
year = {2009},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
booktitle = {Proceedings of the 32nd International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {640–641},
numpages = {2},
location = {Boston, MA, USA},
series = {SIGIR '09}
}

@inproceedings{scholer17,
author = {Thomas, Paul and Scholer, Falk and Bailey, Peter and Moffat, Alistair},
title = {Tasks, Queries, and Rankers in Pre-Retrieval Performance Prediction},
year = {2017},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
booktitle = {Proceedings of the 22nd Australasian Document Computing Symposium},
articleno = {11},
numpages = {4},
location = {Brisbane, QLD, Australia},
series = {ADCS 2017}
}

@inproceedings{passageqpp21,
author = {Sarwar, Ghulam and O’Riordan, Colm},
title = {Passage Based Answer-Set Graph Approach for Query Performance Prediction},
year = {2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
booktitle = {Proceedings of the 26th Australasian Document Computing Symposium},
numpages = {6},
location = {Brisbane, QLD, Australia},
series = {ADCS 2021}
}

==> src/abstract.tex <==
\label{abstract}

A query performance predictor estimates the retrieval effectiveness of an IR system for a given query. An important characteristic of QPP evaluation is that,
since the ground truth retrieval effectiveness for QPP evaluation can be measured with different metrics, %such as AP or nDCG employing different rank cut-off values on document lists retrieved with different IR similarity functions, 
the ground truth itself is not absolute, which is in contrast to other retrieval tasks, such as that of ad-hoc retrieval. Motivated by this argument, the objective of this paper is to investigate how such variances in the ground truth for QPP evaluation can affect the outcomes of QPP experiments. We consider this not only in terms of the absolute values of the evaluation metrics being reported (e.g. Pearson's $r$, Kendall's $\tau$), but also with respect to the changes in the ranks of different QPP systems when ordered by the QPP metric scores.
%(arranged by the QPP evaluation metric values).
Our experiments reveal that the observed QPP outcomes can vary considerably, both in terms of the absolute evaluation metric values and also in terms of the relative system ranks. Through our analysis, we report the optimal combinations of QPP evaluation metric and experimental settings that are likely to lead to smaller variations in the observed results. 

%The evaluation of a QPP method makes use of manually assessed relevance judgments to benchmark different QPP methods on standard IR datasets. The predicted output from a QPP method for any input query is expected to exhibit a high correlation with a retrieval effectiveness evaluation measure, e.g. AP or nDCG. 


==> src/introduction.tex <==
The problem of \emph{query performance prediction} (QPP)
\cite{croft_qpp_sigir02,kurland_tois12,wig_croft_SIGIR07}
has attracted the attention of the Information Retrieval (IR) community over a number of years. QPP involves estimating the retrieval quality of an IR system \emph{without using any relevance assessments or user feedback}~\cite{qpp_dist_IR_sigir05}. More simply, QPP aims to predict how easy or difficult a given query is for an IR system. A diverse range of pre-retrieval (e.g. avgIDF \cite{survey_preret_qpp}) and post-retrieval approaches (e.g. WIG \cite{wig_croft_SIGIR07}, NQC \cite{kurland_tois12}, UEF \cite{uef_kurland_sigir10}) have been proposed for the task of QPP over the years.
% 
% \todo{This para is probably not required here.} Although the working methodology of an unsupervised QPP method itself does not require the presence of manually-assessed relevance judgments for the estimation of query difficulty, the \emph{quantitative evaluation} of QPP methods do, in fact, rely on relevance judgments for the purpose of evaluating different QPP methods on benchmark datasets.
% 
The output of a QPP method, given a query and an IR system, is a real-valued predicted score that is an indication of the predicted retrieval effectiveness of an IR system for the query, i.e., a higher score indicates a better retrieval effectiveness. In this sense, the predicted output from a QPP method for a query should exhibit a high correlation with a retrieval effectiveness evaluation measure, e.g. AP or nDCG \cite{ndcg}.
A standard way of QPP evaluation is thus to compute the agreements between the predicted outputs and a target IR metric (e.g., AP or nDCG) for a query.
%
The values of an IR effectiveness metric for each query thus serve as a set of \emph{reference values} against which the QPP predictions obtained with a particular method can be evaluated. It is important to note that these reference values in QPP evaluation are not \emph{absolute} (akin to the manual relevance assessments), but rather are subject to potentially substantial variations. This is due to the differences in how these reference values are computed via different metrics or on different retrieval models.
Specifically, the computation of an IR metric itself depends on a number of different factors:
\begin{compactitem}
\item \textbf{IR evaluation metric:} This is used to measure the reference values of the retrieval effectiveness (e.g. AP, nDCG etc.).
\item \textbf{IR model:} Variations in the retrieval model may cause significant changes in the positions of the documents retrieved. This can result in variations in the values of the target metric. For instance, the AP of a query computed on a document list retrieved with BM25 may substantially be different from that retrieved with LM-Dirichlet.
\item \textbf{Rank cut-off:} The choice of the ranked list cut-off on which retrieval effectiveness is to be measured (e.g. AP@10 vs. AP@100 etc.) results in different values. Consequently, the measured effectiveness of QPP systems can also vary. A high cut-off value is useful for a recall-oriented task, such as patent retrieval \cite{TakakiFI04,Xue,Ganguly}, whereas a low cut-off caters to a precision-oriented one, such as in web search \cite{pmlr-v15-ravikumar11a,colbert_sigir20}.
\end{compactitem}

A standard way to evaluate QPP is to either measure the correlation between the predicted and the reference values of the retrieval effectiveness (e.g., AP@100 or nDCG@10), or to measure the correlation between the ranks of these values. 
However, variations in each of the aforementioned settings of measuring the ground-truth retrieval effectiveness values can lead to differences in these correlations, potentially either for the values themselves or between their ordinals.
This, in turn, can lead to both differences in the absolute values of reported QPP evaluation measures (e.g., the $\rho$ value for NQC \cite{kurland_tois12} measured with AP@100 as the target metric and LM-Dirichlet as the retrieval model can substantially be different from those measured with AP@1000 as the target metric and BM25 as the retrieval model on the same set of queries), and also in the relative comparison between a number of different QPP measures (e.g., NQC turning out to be better than WIG with AP@100, whereas WIG outperforming NQC when QPP effectiveness is measured with nDCG@10).
%
Such variations can lead to difficulties in reproducing QPP results, both at the level of the correlation values being reported and also in terms of the relative performance of the different competing methods on standard datasets.
%
%changing the reference values of the measured retrieval effectiveness, and can also change the ground-truth relative order of the difficulty of a set of queries.
%This potential instability in the ground-truth for QPP is likely to lead to instability in the relative effectiveness of different QPP approaches.
%
%TODO: Also mention about the relative comparisons between studies.
%

%\para{Our Contributions}
\para{Contributions}
In this paper, we conduct a range of experiments to analyze the potential variations in QPP effectiveness results under different experimental conditions. Specifically, we consider different combinations of IR metric, IR model, and rank cut-off values. The experiments described in Section \ref{sec:res} reveal that the results of QPP do largely depend on these settings. The important implication of our findings is that it may be difficult to reproduce experiments without a precise description of the experimental context.
%TODO: Maybe move this later?
Despite variations in other factors, such as the choice of indexing implementation and set of pre-processing steps, we recommend that a precise description of QPP experimental settings should be followed as a guideline to reduce variations in  reported results.

%DG: reformulated this...
%the conclusions drawn from QPP experiments without a precise description of these settings should be subject to reproducibility concerns. Based on our findings, we also suggest a set of initial conditions as a set of guidelines for future research in QPP. Following these guidelines in future QPP research will likely exhibit overall low variances in the reported results due to other uncontrollable factors, such as the indexing implementation used, pre-processing etc.

%\para{Our Contributions}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main_llncs.tex"
%%% End:


==> src/qpp_eval.tex <==
\label{sec:qppeval}

\subsection{Variations in Ground-truth}

An IR metric mechanism has two key components -- a) the evaluation function itself, which is one of a set of standard measures such as
\texttt{AP}, \texttt{recall}, \texttt{nDCG} etc., and b) a cut-off rank, $k \in \mathbb{Z}$, used to specify the set of retrieved documents to be evaluated, e.g. \texttt{AP@100}, \texttt{precision@5}, \texttt{nDCG@10} etc. We denote an IR function with the notation $\mu_k$, where $\mu \in \mathcal{M}$ denotes a specific function from a universal set, $\mathcal{M}$, of such available functions, and $k$ (the cut-off rank) denotes a particular \emph{instance} of $\mu$ (note that different values of $k$ may lead to different results even using the same function, e.g. the values of \texttt{AP@100} and \texttt{AP@200} are most likely to be different).

Formally speaking, if a QPP function $\phi$ predicts a score reflecting the likelihood of effective retrieval of the form $\phi: q \mapsto \mathbb{R}$, and if $\mu^k(q)$ denotes the IR effectiveness measure of $q$, then the overall QPP effectiveness for a set of queries is given by
\begin{equation}
r(\phi, Q, \mu_k) =
\rho(
\{\phi(q_1),\ldots,\phi(q_n)\},
\{\mu(q_1),\ldots,\mu(q_n)\}
),    \label{eq:qppreward}
\end{equation}
where, $Q=\{q_1,\ldots,q_n\}$ is a set of $n$ benchmark queries, and $\rho: \mathbb{R}^n \times \mathbb{R}^n \mapsto \mathbb{R}$ is a correlation measure between two (ordered) sets of values, each of cardinality $n$. Examples of correlation functions include Pearson's correlation $\rho_p$, Spearman's correlation $\rho_s$, Kendall's $\tau$ etc. 

It is evident from Equation \ref{eq:qppreward} that the value of the QPP effectiveness, $r(\phi,Q,\mu_k)$ measured with a particular correlation function such as Pearson's $\rho_p$, of a QPP method $\phi$ for a set of queries $Q$ depends on both the
choice of the function $\mu \in \mathcal{M}$ (e.g. $\mu$ being one of \texttt{AP}, \texttt{nDCG} etc.)
and the cut-off $k$ used to construct the ground-truth for evaluation.
Consequently, the relative effectiveness of various QPP methods, e.g. NQC \cite{kurland_tois12}, WIG \cite{wig_croft_SIGIR07}, UEF \cite{uef_kurland_sigir10} etc., may in fact depend on the choices of these parameters, i.e., whether to use AP or P@k as the evaluation metric, whether to use top-100 documents for computing AP or to use top-5 documents for computing the precision of the top-retrieved set etc.

%(e.g. the study \cite{hamed_neuralqpp} used both AP@1000 and nDCG@20).
%first use a \emph{target IR metric}  to sort a set of benchmark queries in decreasing order of these values. Similarly, as a second step, the predicted values are  

However, somewhat surprisingly, there exists no study investigating the effects of relative changes in the order of the effectiveness of QPP systems akin to studies that investigate the relative changes in the ranks of retrieval systems with variations in the pool depth and the metrics used for evaluation \cite{maip_cikm,zobel_cikm09}.
While most studies on QPP uses average precision for constructing the ground-truth \cite{uef_kurland_sigir10,kurland_tois12}, some of them explicitly mention the number of top-retrieved documents used, whereas the others do not mention this cut-off explicitly as a part of describing their experiment setup \cite{wig_croft_SIGIR07}. Further, some studies used two different metrics to report the relative effectiveness across different QPP systems, e.g. \cite{wig_croft_SIGIR07} used both AP and MRR, whereas \cite{hamed_neuralqpp} used AP and nDCG@20. 

It is evident from existing research that there is no consensus among IR researchers on the prescribed choices of the metric to employ or the cut-off rank to use for the purpose of measuring QPP of various methods in a reproducible manner. The primary motivation of this paper is to investigate these research questions towards 


% \subsection{Generalized Metric to Measure Correlation among Multiple Ranked List of Queries}
% % To estimate the specificity of queries, we measure the correlation coefficient (i.e. Pearsons's $\mathalpha{r}$ / Spearman's $\rho$ / Kendall's $\tau$) between a predicted order of queries obtained by a post-retrieval QPP measure, such as NQC, WIG or Clarity, and the rank induced by a retrieval evaluation measure, like AP, nDCG, Recall, MRR etc.
% % in practice. The higher the correlation coefficient (tending to $+1$), more reliable the retrieval evaluation metric is. However, in our investigation for \textbf{RQ1}, we aim to observe if there is any significant variations in the relative effectiveness of QPP methods, which leads us to measure the overall deviation of the ranks of any particular query in a number of obtained ranked lists (let's say, one predicted list comes from NQC and there are $3$ other ranked list for the same set of queries obtained by \texttt{AP@100, Recall@1000 and Precision@10}). Therefore, for a given query, we measure the perturbation (or absolute difference) of the ranks across all the ordered lists.

% \paragraph{\textbf{Metric 1.}} 
% Let us assume that we want to estimate the perturbation of queries, $q_1, q_2, \ldots, q_m$, across $n$ number of ordered list, say $L_1$ (obtained by NQC), $L_2$ (ranked using $AP@1000$), $L_3$ (ordered list by $Recall@1000$), \ldots, $L_n$; and the rank of $q$ at any ranked list $L_i$ is denoted as $r(q,L_i)$. Therefore, the overall perturbation $\mathcal{P}$ of the query $q$ can be measured as  
% \begin{equation}
%     \mathcal{P} = 1 - \sum_{x=1}^{m} \sum_{i=1}^{n-1} \sum_{j=i+1}^{n} \frac{1}{|L_i|=|L_j|}|r(q_x,L_i) - r(q_x, L_j)|
%     \label{eq:absdiff}
% \end{equation}
% % According to \textbf{RQ1}, the more the value of $\mathcal{P}$ is close to $0$, i.e. a small absolute difference among paired up ranked lists, more stable the retrieval evaluation measures are.
% % Hence, we define a generalized metric $\mathcal{X}$ to measure the correlation among multiple retrieval evaluation measures for any random query $q$ taking the overall perturbation into account as
% % \begin{equation}
% %     \mathcal{X} = 1 - \mathcal{P}/\mathcal{N}
% %     \label{eq:perturb}
% % \end{equation}
% % % 
% % where, $\mathcal{N}$ = max($|r(q,L_i) - r(q, L_j)|_{i=1, \ldots, n-1; j=i+1, \ldots, n}$)
% % Clearly, the range of the metric $\mathcal{X}$ lies in $[0,1]$ and the larger $\mathcal{X}$ indicates more stability across retrieval evaluation metrics which eventually leads us to the conclusion for a given query $q$ that irrespective of the ground truths (i.e. retrieval evaluation measures), the specificity of $q$ is invariant. 

% \paragraph{\textbf{Metric 2.}} Instead of measuring absolute differences across multiple ranked lists, we incorporate \emph{Kendall's distance} to capture overall deviation. Adding Kendall's distance in place of absolute difference in Equation \ref{eq:absdiff}, we obtain
% \begin{equation}
%     \mathcal{X} = \sum_{i=1}^{n-1} \sum_{j=i+1}^{n}\mathcal{K}(L_i, L_j)
%     \label{eq:kendaldist}
% \end{equation}
% % 
% where, $\mathcal{K}(L_i, L_j) = |(x,y):x<y,(L_i(x) < L_i(y) \wedge L_j(x) > L_j(y))   \vee$ 
% $(L_i(x) > L_i(y) \wedge L_j(x) < L_j(y))|$

==> tables/contingency_rho.tex <==
\begin{table}[ht]
\centering
\begin{adjustbox}{width=1\textwidth}

\begin{tabular}{@{}l@{~~}l@{~~}l@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c}

\toprule
& & & \multicolumn{8}{c}{$K-\tau(i,j)$} \\

\cmidrule{4-11}

& Metric & Ret. Model & 
AP & AP & 
Recall & Recall & Recall & 
nDCG & nDCG & nDCG \\

& & & 
@100 & @1000 & 
@10 & @100 & @1000 & 
@10 & @100 & @1000 \\

\midrule

& AP@10 & BM25 & 
1.0000 & 0.8095 & 
1.0000 & 0.9048 & 0.6190 &
1.0000 & 1.0000 & 0.6190 \\

& & LM-Dir & 
0.9048 & 0.8095 & 
1.0000 & 1.0000 & 0.8095 &
1.0000 & 0.9048 & 0.7143 \\

\cmidrule{2-3}

& AP@100 & BM25 & 
\nores & 0.8095 & 
1.0000 & 0.9048 & 0.6190 &
1.0000 & 1.0000 & 0.6190 \\

& & LM-Dir & 
\nores & 0.9048 & 
0.9048 & 0.9048 & 0.7143 &
0.9048 & 1.0000 & 0.8095 \\

\cmidrule{2-3}

& AP@1000 & BM25 & 
\nores & \nores & 
0.8095 & 0.7143 & 0.6190 &
0.8095 & 0.8095 & 0.8095 \\

& & LM-Dir & 
\nores & \nores & 
0.8095 & 0.8095 & 0.8095 &
0.8095 & 0.9048 & 0.9048 \\

\cmidrule{2-3}

& Recall@10 & BM25 & 
\nores & \nores & 
\nores & 0.9048 & 0.6190 &
1.0000 & 1.0000 & 0.6190 \\

& & LM-Dir & 
\nores & \nores & 
\nores & 1.0000 & 0.8095 &
1.0000 & 0.9048 & 0.7143 \\

\cmidrule{2-3}

$S-\rho$ & Recall@100 & BM25 & 
\nores & \nores & 
\nores & \nores & 0.7143 &
0.9048 & 0.9048 & 0.5238 \\

& & LM-Dir & 
\nores & \nores & 
\nores & \nores & 0.8095 &
1.0000 & 0.9048 & 0.7143 \\

\cmidrule{2-3}

& Recall@1000 & BM25 & 
\nores & \nores & 
\nores & \nores & \nores &
0.6190 & 0.6190 & 0.8095 \\

& & LM-Dir & 
\nores & \nores & 
\nores & \nores & \nores &
0.8095 & 0.7143 & 0.9048 \\

\cmidrule{2-3}

& nDCG@10 & BM25 & 
\nores & \nores & 
\nores & \nores & \nores &
\nores & 1.0000 & 0.6190 \\

& & LM-Dir & 
\nores & \nores & 
\nores & \nores & \nores &
\nores & 0.9048 & 0.7143 \\

\cmidrule{2-3}

& nDCG@100 & BM25 & 
\nores & \nores & 
\nores & \nores & \nores &
\nores & \nores & 0.6190 \\

& & LM-Dir & 
\nores & \nores & 
\nores & \nores & \nores &
\nores & \nores & 0.8095 \\


\bottomrule
\end{tabular}
\end{adjustbox}
%}
\caption{Contingency table}
\label{tab:contrho}
\end{table}

==> tables/sd.tex <==
\begin{table}[ht]
\centering
\begin{adjustbox}{width=1\textwidth}
% \small

\begin{tabular}{@{}l@{~~}l@{~~}l@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c}

\toprule
& & & & \multicolumn{4}{c}{Retrieval Evaluation Metric} &  
\\ 

\cmidrule{5-8}

QPP Model & & IR Model & & AP@100 & nDCG@100 & Recall@100 & P@10 & 
\\

\midrule

& & & & & & & & $\sigma_{metric}$ \\
& & LM-JM & & 0.3795 & 0.3966 & 0.3869 & 0.3311 & \textbf{0.0291} \\
& \textbf{$r$} & BM25 & & 0.5006 & 0.4879 & 0.4813 & 0.2525 & 0.1190 \\
& & LM-Dir & & 0.5208 & 0.5062 & 0.4989 & 0.2851 & 0.1121 \\
\cmidrule{5-8}
AvgIDF & & & $\sigma_{model}$ & 0.0764 & 0.0587 & 0.0602 & \textbf{0.0395} \\

\cmidrule{2-9}

% & & BM25 & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% AvgIDF& \textbf{$P-r$} & LM-Dir & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% & & LM-JM & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% \cmidrule{5-8}
% & & & $\sigma_{model}^2$ & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\

% \cmidrule{2-9}

& & & & & & & & $\sigma_{metric}$ \\
& & LM-JM & & 0.3175 & 0.3285 & 0.3278 & 0.2193 & \textbf{0.0529} \\
& \textbf{$\tau$} & BM25 & & 0.3144 & 0.3162 & 0.3319 & 0.2040 & 0.0589 \\
& & LM-Dir & & 0.3307 & 0.3407 & 0.3440 & 0.2155 & 0.0617 \\
\cmidrule{5-8}
& & & $\sigma_{model}$ & 0.0087 & 0.0123 & \textbf{0.0084} & 0.0123 \\

\midrule
\midrule

% ================================================

& & & & & & & & $\sigma_{metric}$ \\
& & LM-JM & & 0.3652 & 0.4169 & 0.4503 & 0.2548 & 0.0855 \\
& \textbf{$r$} & BM25 & & 0.3563 & 0.4118 & 0.4495 & 0.2707 & \textbf{0.0777} \\
& & LM-Dir & & 0.4354 & 0.4583 & 0.4854 & 0.2842 & 0.0901 \\
\cmidrule{5-8}
NQC & & & $\sigma_{model}$ & 0.0433 & 0.0255 & 0.0205 & \textbf{0.0147} \\

\cmidrule{2-9}

% & & BM25 & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% NQC & \textbf{$P-r$} & LM-Dir & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% & & LM-JM & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% \cmidrule{5-8}
% & & & $\sigma_{model}^2$ & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\

% \cmidrule{2-9}

& & & & & & & & $\sigma_{metric}$ \\
& & LM-JM & & 0.3100 & 0.3319 & 0.3657 & 0.2061 & 0.0688 \\
& \textbf{$\tau$} & BM25 & & 0.3170 & 0.3370 & 0.3551 & 0.2374 & \textbf{0.0519} \\
& & LM-Dir & & 0.3539 & 0.3713 & 0.3828 & 0.2379 & 0.0668 \\
\cmidrule{5-8}
& & & $\sigma_{model}$ & 0.0236 & 0.0214 & \textbf{0.0140} & 0.0182 \\

\midrule
\midrule

% ==========================================

& & & & & & & & $\sigma_{metric}$ \\
& & LM-JM & & 0.4056 & 0.4071 & 0.3971 & 0.3054 & \textbf{0.0491} \\
& & BM25 & & 0.4488 & 0.4563 & 0.4386 & 0.3485 & 0.0502 \\
& \textbf{$r$} & LM-Dir & & 0.4908 & 0.4798 & 0.4632 & 0.3423 & 0.0688 \\
\cmidrule{5-8}
WIG & & & $\sigma_{model}$ & 0.0426 & 0.0371 & 0.0334 & \textbf{0.0233} \\

\cmidrule{2-9}

% & & BM25 & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% WIG & \textbf{$P-r$} & LM-Dir & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% & & LM-JM & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% \cmidrule{5-8}
% & & & $\sigma_{model}^2$ & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\

% \cmidrule{2-9}

& & & & & & & & $\sigma_{metric}$ \\
& & LM-JM & & 0.2514 & 0.2567 & 0.2607 & 0.2209 & \textbf{0.0181} \\
& \textbf{$\tau$} & BM25 & & 0.3116 & 0.3181 & 0.3125 & 0.2549 & 0.0297 \\
& & LM-Dir & & 0.3194 & 0.3267 & 0.3259 & 0.2493 & 0.0375 \\
\cmidrule{5-8}
& & & $\sigma_{model}$ & 0.0372 & 0.0382 & 0.0344 & \textbf{0.0182} \\

\midrule
\midrule

% ======================================

& & & & & & & & $\sigma_{metric}$ \\
& & LM-JM & & 0.4746 & 0.4763 & 0.4646 & 0.3573 & \textbf{0.0575} \\
& \textbf{$r$} & BM25 & & 0.5386 & 0.5476 & 0.5263 & 0.4182 & 0.0603 \\
& & LM-Dir & & 0.5693 & 0.5566 & 0.5373 & 0.3971 & 0.0797 \\
\cmidrule{5-8}
UEF(WIG) & & & $\sigma_{model}$ & 0.0483 & 0.0440 & 0.0392 & \textbf{0.0309} \\

\cmidrule{2-9}

% & & BM25 & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% UEF(WIG) & \textbf{$P-r$} & LM-Dir & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% & & LM-JM & & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
% \cmidrule{5-8}
% & & & $\sigma_{model}^2$ & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\

% \cmidrule{2-9}

& & & & & & & & $\sigma_{metric}$ \\
& & LM-JM & & 0.3017 & 0.3080 & 0.3128 & 0.2651 & \textbf{0.0217} \\
& \textbf{$\tau$} & BM25 & & 0.3677 & 0.3754 & 0.3688 & 0.3008 & 0.0351 \\
& & LM-Dir & & 0.3833 & 0.3920 & 0.3911 & 0.2992 & 0.0450 \\
\cmidrule{5-8}
& & & $\sigma_{model}$ & 0.0433 & 0.0445 & 0.0403 & \textbf{0.0202} \\

\bottomrule
\end{tabular}
\end{adjustbox}
%}
\caption{Variance table}
\label{tab:var}
\end{table}

